DQ-DETR: Dual Query Detection Transformer for Phrase Extraction and Grounding

In this paper, we study the problem of visual grounding by considering both phrase extraction and grounding (PEG). In contrast to the previous phrase-known-at-test setting, PEG requires a model to extract phrases from text and locate objects from images simultaneously, which is a more practical setting in real applications. As phrase extraction can be regarded as a $1$D text segmentation problem, we formulate PEG as a dual detection problem and propose a novel DQ-DETR model, which introduces dual queries to probe different features from image and text for object prediction and phrase mask prediction. Each pair of dual queries is designed to have shared positional parts but different content parts. Such a design effectively alleviates the difficulty of modality alignment between image and text (in contrast to a single query design) and empowers Transformer decoder to leverage phrase mask-guided attention to improve performance. To evaluate the performance of PEG, we also propose a new metric CMAP (cross-modal average precision), analogous to the AP metric in object detection. The new metric overcomes the ambiguity of Recall@1 in many-box-to-one-phrase cases in phrase grounding. As a result, our PEG pre-trained DQ-DETR establishes new state-of-the-art results on all visual grounding benchmarks with a ResNet-101 backbone. For example, it achieves $91.04\%$ and $83.51\%$ in terms of recall rate on RefCOCO testA and testB with a ResNet-101 backbone. Code will be availabl at \url{https://github.com/IDEA-Research/DQ-DETR}.

==> images_tex/dual_queries.tex <==
\begin{figure}[th]
% \vspace{-0.6cm}
\centering
\subfigure[ ]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=\linewidth]{images/mdetr_query_text_align_tsne_43.png}
\vspace{-0.8cm}
\label{fig:mdetr_feature_tsne}
\end{minipage}
}%
\subfigure[ ]{
\begin{minipage}[t]{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{images/mdetr_dual_queries_tsne_43.png}
\vspace{-0.8cm}
\label{fig:dmdetr_query_pair}
\end{minipage}
}%
\subfigure[ ]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=\linewidth]{images/bbox_l1_comparison_v2.png}
\vspace{-0.8cm}
\label{fig:compare_bbox_l1}
\end{minipage}
}%
\centering
\vspace{-0.3cm}
\caption{\small{(a) Visualization of query and text features in MDETR~\citep{kamath2021mdetr} by t-SNE. Different colors are for different pairs of features. Some paired features are linked by gray lines for easy check. The ``comp-1'' and ``comp-2'' are the main principal components after dimensionality reduction. Some clustering features are shaded in blue. (b) Visualization of dual queries in our DQ-DETR by t-SNE. Different colors are for different pairs of dual queries. (c) Comparison of test bounding box L1 loss vs. training epochs. (Best viewed in color.) }
% \shilong{Enlarge the images. explain the comp-1\&2. add a cls. losses comparison.}
% \hangx{the fontsize in the figure is too small}
}
% \vspace{-0.1cm}
\end{figure}


==> tables_tex/pretrain.tex <==
\begin{table}[ht]
\begin{center}
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllll}
\shline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} &\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Epoches}}} &  \multicolumn{3}{l}{\textbf{Flickr30k}} & \textbf{GQA}         \\
\multicolumn{1}{c}{} &       & CMAP$_{50}$    & AP$_{50}$ & R@1 & AP$_{50}$ \\
\shline
OFA-REC+spaCy & - & 15.8 & - & - & - \\
\hline
MDETR & 50 & 61.4  & 75.6 & 82.5 & 58.9\\
\hline
DQ-DETR (Ours) & \textbf{25}  & \textbf{67.9} \small{\red{(+6.5)}} & \textbf{78.7} \small{\red{(+2.1)}} & \textbf{83.2}\small{\red{(+0.7)}} & \textbf{60.0} \small{\red{(+1.1)} }\\
\shline
\end{tabular}}
\vspace{0.1cm}
\caption{
Pre-training result comparisons with two baselines: OFA-REC+spaCy~\cite{PengWang2022UNIFYINGAT, spacy2} and MDETR~\cite{kamath2021mdetr}. The numbers in brackets are the gains between DQ-DETR and MDETR.  All models are pre-trained with a ResNet-101 backbone. Note that OFA-REC is trained for REC with about 50M pre-train images, which is much larger than our 200k images.
}
\vspace{-0.2cm}
\label{tab:pretrain}
\end{center}
\end{table}
